MDroid+: A Mutation Testing Framework for Android

Mutation testing has shown great promise in assessing the effectiveness of test suites while exhibiting additional applications to test-case generation, selection, and prioritization. Traditional mutation testing typically utilizes a set of simple language specific source code transformations, called operators, to introduce faults. However, empirical studies have shown that for mutation testing to be most effective, these simple operators must be augmented with operators specific to the domain of the software under test. One challenging software domain for the application of mutation testing is that of mobile apps. While mobile devices and accompanying apps have become a mainstay of modern computing, the frameworks and patterns utilized in their development make testing and verification particularly difficult. As a step toward helping to measure and ensure the effectiveness of mobile testing practices, we introduce MDroid+, an automated framework for mutation testing of Android apps. MDroid+ includes 38 mutation operators from ten empirically derived types of Android faults and has been applied to generate over 8,000 mutants for more than 50 apps.

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }



\newcommand\ROCCO[1]{\textcolor{blue}{\nb{ROCCO}{#1}}}
\newcommand\MAX[1]{\textcolor{blue}{\nb{MAX}{#1}}}
\newcommand\GABRIELE[1]{\textcolor{blue}{\nb{GABRIELE}{#1}}}
\newcommand\DENYS[1]{\textcolor{blue}{\nb{DENYS}{#1}}}
\newcommand\MARIO[1]{\textcolor{blue}{\nb{MARIO}{#1}}}
\newcommand\CARLOS[1]{\textcolor{blue}{\nb{CARLOS}{#1}}}
\newcommand\CHRIS[1]{\textcolor{blue}{\nb{CHRIS}{#1}}}

\newcommand\NEW[1]{\nb{NEW}{#1}}





